Mobile Manipulation Instruction Generation from Multiple Images with Automatic Metric Enhancement

We consider the problem of generating free-form mobile manipulation instructions based on a target object image and receptacle image. Conventional image captioning models are not able to generate appropriate instructions because their architectures are typically optimized for single-image. In this study, we propose a model that handles both the target object and receptacle to generate free-form instruction sentences for mobile manipulation tasks. Moreover, we introduce a novel training method that effectively incorporates the scores from both learning-based and n-gram based automatic evaluation metrics as rewards. This method enables the model to learn the co-occurrence relationships between words and appropriate paraphrases. Results demonstrate that our proposed method outperforms baseline methods including representative multimodal large language models on standard automatic evaluation metrics. Moreover, physical experiments reveal that using our method to augment data on language instructions improves the performance of an existing multimodal language understanding model for mobile manipulation.

==> tab/error-3.tex <==
\begin{figure}[t]
  \centering
  \begin{minipage}[b]{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig/error/error3_tar.jpg}
    \caption*{(a)}
    \label{fig:target_image}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig/error/error3_dest.jpg}
    \caption*{(b)}
  \end{minipage}
  \begin{tabular}{|p{0.9\linewidth}|}
    \hline
    \textbf{Ref:} ``pick up white curtain to the kitchen'' \\
    \hline
    \textbf{Generated Sentence:} ``pick up the lamp beside the bed and move it to the kitchen'' \\
    \hline
  \end{tabular}
  \caption{An example of a case of discrepancies in the objects of interest. (a) Target object image and (b) receptacle image.}
  \label{fig:error-3}
  \vspace{-3mm}
\end{figure}

==> tab/error.tex <==
\begin{table}[t]
    \caption{\small Categorization of failure cases.}
    \normalsize
    \centering
    \begin{tabular}{l@{\hspace{2mm}}c@{\hspace{2mm}}}
        \toprule
        Error type & \textit{\# $\mathrm{Samples}$ }\\
        \midrule
        Errors in detailed information & 27 \\
        Severe errors regarding objects/locations & 26 \\
        Discrepancies in object of interest & 19 \\
        Ambiguous instruction & 3 \\
        \midrule
        Total & 75 \\
        \bottomrule
    \end{tabular}
    \label{tab:error}
\end{table}


==> tab/params.tex <==
% \begin{table}[t]
%     \normalsize
%     \centering
%     \caption{\small Experimental settings of the proposed method.}
%     \label{tab:params}
%     \begin{tabular}{ll}
%         \toprule
%         Optimizer & AdamW ($\beta_1=0.9$, $\beta_2=0.99$) \\
%         \hline
%         Beam size & $3$ \\
%         \hline
%         \vspace{1mm}
%         Beam length & $30$ \\
%         \hline
%         \multirow{3}{*}{Learning rate} & TQPP: $1.0\times10^{-4}$ \\
%                                        & PDMP: $1.0\times10^{-4}$ \\
%                                        & HCCP: $5.0\times10^{-6}$ \\
%         \hline
%         \multirow{3}{*}{Batch size}    & TQPP: $32$ \\
%                                        & PDMP: $32$ \\
%                                        & HCCP: $2$ \\
%         \hline
%         \multirow{3}{*}{Epoch}       & TQPP: $100$ \\
%                                        & PDMP: $100$ \\
%                                        & HCCP: $8$ \\
%         \hline
%         \multirow{3}{*}{Reward weights} & $\lambda_1$: $0.25$ \\
%                                        & $\lambda_2$: $0.25$ \\
%                                        & $\lambda_3$: $0.5$ \\
%         \bottomrule
%     \end{tabular}
% \end{table}


==> tab/physical-model.tex <==
\begin{figure}[t]
  \centering
  \begin{minipage}[b]{\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth]{fig/setting/physical-modelv2.png}
  \end{minipage}
  \hfill
  \vspace{-2mm}
  \caption{Experimental environment\cite{wrs2020} and the robot platform\cite{yamamoto2019development} used for the physical experiments.}
  \label{fig:physical-model}
  \vspace{-5mm}
\end{figure}
